United we stand, Divided we fall: Handling Weak Complementary Relationships for Audio-Visual Emotion Recognition in Valence-Arousal Space

Audio and visual modalities are two predominant contact-free channels in videos, which are often expected to carry a complementary relationship with each other. However, they may not always complement each other, resulting in poor audio-visual feature representations. In this paper, we introduce Gated Recursive Joint Cross Attention (GRJCA) using a gating mechanism that can adaptively choose the most relevant features to effectively capture the synergic relationships across audio and visual modalities. Specifically, we improve the performance of Recursive Joint Cross-Attention (RJCA) by introducing a gating mechanism to control the flow of information between the input features and the attended features of multiple iterations depending on the strength of their complementary relationship. For instance, if the modalities exhibit strong complementary relationships, the gating mechanism emphasizes cross-attended features, otherwise non-attended features. To further improve the performance of the system, we also explored a hierarchical gating approach by introducing a gating mechanism at every iteration, followed by high-level gating across the gated outputs of each iteration. The proposed approach improves the performance of RJCA model by adding more flexibility to deal with weak complementary relationships across audio and visual modalities. Extensive experiments are conducted on the challenging Affwild2 dataset to demonstrate the robustness of the proposed approach. By effectively handling the weak complementary relationships across the audio and visual modalities, the proposed model achieves a Concordance Correlation Coefficient (CCC) of 0.561 (0.623) and 0.620 (0.660) for valence and arousal respectively on the test set (validation set).

==> Competition/0_abstract.tex <==
\begin{abstract}
Multimodal emotion recognition has recently drawn a lot of interest in affective computing as it has immense potential to outperform isolated unimodal approaches. %Though multiple modalities are often expected to be complementary with each other, they may also exhibit contradictory relationship which may result in poor multimodal feature representations, thereby degrading the performance of the system.  
Audio and visual modalities are two predominant contact-free channels in videos, which are often expected to carry a complementary relationship with each other. However, audio and visual channels may not always be complementary with each other, resulting in poor audio-visual feature representations, thereby degrading the performance of the system.   
%Effectively leveraging the intra and inter-modal relationships among audio and visual modalities plays a crucial role to obtain robust multimodal feature representations and improve the overall accuracy of ER. 
In this paper, we propose a flexible audio-visual fusion model that can adapt to weak complementary relationships using a gated attention mechanism. %, where the attended features obtained from the 
%recursive joint cross attention model are selected only when the audio and visual modalities exhibit a strong complementary relationship with each other. 
Specifically, we extend the recursive joint cross-attention model by introducing gating mechanism in every iteration to control the flow of information between the input features and the attended features depending on the strength of their complementary relationship. For instance, if the modalities exhibit strong complementary relationships, the gating mechanism chooses cross-attended features, otherwise non-attended features. To further improve the performance of the system, we further introduce stage gating mechanism, which is used to control the flow of information across the gated outputs of each iteration.   
%a gating mechanism is designed to learn the contribution of the recursive cross-joint attention mechanism, which allows us to adaptively select the attended or non-attended features based on the strong or weak complementary relationship with each other respectively. 
Therefore, the proposed model improves the performance of the system even when the audio and visual modalities do not have a strong complementary relationship with each other by adding more flexibility to the recursive joint cross attention mechanism. %In order to further enhance the feature representations, we have explored transformers to effectively capture the temporal dynamics of the audio-visual feature representations.
%a recursive joint cross-attention model is proposed along with transformers to exploit the inter-modal complementary relationships as well as intra modal temporal dependencies. In particular, we explore the prospect of obtaining more refined feature representations for audio and visual modalities by iteratively refining the features in a recursive fashion. In addition to that, we have explored transformers to efficiently capture the temporal dynamics among the obtained audio-visual feature representations. By effectively capturing the complementary inter-modal relationships and semantic temporal relationships, the proposed model significantly outperforms the state-of-the-art methods. 
The proposed model has been evaluated on the challenging Affwild2 dataset and significantly outperforms the state-of-the-art fusion approaches. 
\end{abstract}

==> Competition/1_intro.tex <==
\section{Introduction}
\label{sec:intro}

Please follow the steps outlined below when submitting your manuscript to the IEEE Computer Society Press.
This style guide now has several important modifications (for example, you are no longer warned against the use of sticky tape to attach your artwork to the paper), so all authors should read this new version.

%-------------------------------------------------------------------------
\subsection{Language}

All manuscripts must be in English.

\subsection{Dual submission}

Please refer to the author guidelines on the \confName\ \confYear\ web page for a
discussion of the policy on dual submissions.

\subsection{Paper length}
Papers, excluding the references section, must be no longer than eight pages in length.
The references section will not be included in the page count, and there is no limit on the length of the references section.
For example, a paper of eight pages with two pages of references would have a total length of 10 pages.
{\bf There will be no extra page charges for \confName\ \confYear.}

Overlength papers will simply not be reviewed.
This includes papers where the margins and formatting are deemed to have been significantly altered from those laid down by this style guide.
Note that this \LaTeX\ guide already sets figure captions and references in a smaller font.
The reason such papers will not be reviewed is that there is no provision for supervised revisions of manuscripts.
The reviewing process cannot determine the suitability of the paper for presentation in eight pages if it is reviewed in eleven.

%-------------------------------------------------------------------------
\subsection{The ruler}
The \LaTeX\ style defines a printed ruler which should be present in the version submitted for review.
The ruler is provided in order that reviewers may comment on particular lines in the paper without circumlocution.
If you are preparing a document using a non-\LaTeX\ document preparation system, please arrange for an equivalent ruler to appear on the final output pages.
The presence or absence of the ruler should not change the appearance of any other content on the page.
The camera-ready copy should not contain a ruler.
(\LaTeX\ users may use options of \texttt{cvpr.sty} to switch between different versions.)

Reviewers:
note that the ruler measurements do not align well with lines in the paper --- this turns out to be very difficult to do well when the paper contains many figures and equations, and, when done, looks ugly.
Just use fractional references (\eg, this line is $087.5$), although in most cases one would expect that the approximate location will be adequate.


\subsection{Paper ID}
Make sure that the Paper ID from the submission system is visible in the version submitted for review (replacing the ``*****'' you see in this document).
If you are using the \LaTeX\ template, \textbf{make sure to update paper ID in the appropriate place in the tex file}.


\subsection{Mathematics}

Please number all of your sections and displayed equations as in these examples:
\begin{equation}
  E = m\cdot c^2
  \label{eq:important}
\end{equation}
and
\begin{equation}
  v = a\cdot t.
  \label{eq:also-important}
\end{equation}
It is important for readers to be able to refer to any particular equation.
Just because you did not refer to it in the text does not mean some future reader might not need to refer to it.
It is cumbersome to have to use circumlocutions like ``the equation second from the top of page 3 column 1''.
(Note that the ruler will not be present in the final copy, so is not an alternative to equation numbers).
All authors will benefit from reading Mermin's description of how to write mathematics:
\url{http://www.pamitc.org/documents/mermin.pdf}.

\subsection{Blind review}

Many authors misunderstand the concept of anonymizing for blind review.
Blind review does not mean that one must remove citations to one's own work---in fact it is often impossible to review a paper unless the previous citations are known and available.

Blind review means that you do not use the words ``my'' or ``our'' when citing previous work.
That is all.
(But see below for tech reports.)

Saying ``this builds on the work of Lucy Smith [1]'' does not say that you are Lucy Smith;
it says that you are building on her work.
If you are Smith and Jones, do not say ``as we show in [7]'', say ``as Smith and Jones show in [7]'' and at the end of the paper, include reference 7 as you would any other cited work.

An example of a bad paper just asking to be rejected:
\begin{quote}
\begin{center}
    An analysis of the frobnicatable foo filter.
\end{center}

   In this paper we present a performance analysis of our previous paper [1], and show it to be inferior to all previously known methods.
   Why the previous paper was accepted without this analysis is beyond me.

   [1] Removed for blind review
\end{quote}


An example of an acceptable paper:
\begin{quote}
\begin{center}
     An analysis of the frobnicatable foo filter.
\end{center}

   In this paper we present a performance analysis of the  paper of Smith \etal [1], and show it to be inferior to all previously known methods.
   Why the previous paper was accepted without this analysis is beyond me.

   [1] Smith, L and Jones, C. ``The frobnicatable foo filter, a fundamental contribution to human knowledge''. Nature 381(12), 1-213.
\end{quote}

If you are making a submission to another conference at the same time, which covers similar or overlapping material, you may need to refer to that submission in order to explain the differences, just as you would if you had previously published related work.
In such cases, include the anonymized parallel submission~\cite{Authors14} as supplemental material and cite it as
\begin{quote}
[1] Authors. ``The frobnicatable foo filter'', F\&G 2014 Submission ID 324, Supplied as supplemental material {\tt fg324.pdf}.
\end{quote}

Finally, you may feel you need to tell the reader that more details can be found elsewhere, and refer them to a technical report.
For conference submissions, the paper must stand on its own, and not {\em require} the reviewer to go to a tech report for further details.
Thus, you may say in the body of the paper ``further details may be found in~\cite{Authors14b}''.
Then submit the tech report as supplemental material.
Again, you may not assume the reviewers will read this material.

Sometimes your paper is about a problem which you tested using a tool that is widely known to be restricted to a single institution.
For example, let's say it's 1969, you have solved a key problem on the Apollo lander, and you believe that the 1970 audience would like to hear about your
solution.
The work is a development of your celebrated 1968 paper entitled ``Zero-g frobnication: How being the only people in the world with access to the Apollo lander source code makes us a wow at parties'', by Zeus \etal.

You can handle this paper like any other.
Do not write ``We show how to improve our previous work [Anonymous, 1968].
This time we tested the algorithm on a lunar lander [name of lander removed for blind review]''.
That would be silly, and would immediately identify the authors.
Instead write the following:
\begin{quotation}
\noindent
   We describe a system for zero-g frobnication.
   This system is new because it handles the following cases:
   A, B.  Previous systems [Zeus et al. 1968] did not  handle case B properly.
   Ours handles it by including a foo term in the bar integral.

   ...

   The proposed system was integrated with the Apollo lunar lander, and went all the way to the moon, don't you know.
   It displayed the following behaviours, which show how well we solved cases A and B: ...
\end{quotation}
As you can see, the above text follows standard scientific convention, reads better than the first version, and does not explicitly name you as the authors.
A reviewer might think it likely that the new paper was written by Zeus \etal, but cannot make any decision based on that guess.
He or she would have to be sure that no other authors could have been contracted to solve problem B.
\medskip

\noindent
FAQ\medskip\\
{\bf Q:} Are acknowledgements OK?\\
{\bf A:} No.  Leave them for the final copy.\medskip\\
{\bf Q:} How do I cite my results reported in open challenges?
{\bf A:} To conform with the double-blind review policy, you can report results of other challenge participants together with your results in your paper.
For your results, however, you should not identify yourself and should not mention your participation in the challenge.
Instead present your results referring to the method proposed in your paper and draw conclusions based on the experimental comparison to other results.\medskip\\

\begin{figure*}[t]
  \centering
  %\fbox{\rule{0pt}{2in} \rule{0.9\linewidth}{0pt}}
   \includegraphics[width=1.0\linewidth]{ABAW8.png}

   \caption{Example of caption.
   It is set in Roman so that mathematics (always set in Roman: $B \sin A = A \sin B$) may be included without an ugly clash.}
   \label{fig:onecol}
\end{figure*}

\subsection{Miscellaneous}

\noindent
Compare the following:\\
\begin{tabular}{ll}
 \verb'$conf_a$' &  $conf_a$ \\
 \verb'$\mathit{conf}_a$' & $\mathit{conf}_a$
\end{tabular}\\
See The \TeX book, p165.

The space after \eg, meaning ``for example'', should not be a sentence-ending space.
So \eg is correct, {\em e.g.} is not.
The provided \verb'\eg' macro takes care of this.

When citing a multi-author paper, you may save space by using ``et alia'', shortened to ``\etal'' (not ``{\em et.\ al.}'' as ``{\em et}'' is a complete word).
If you use the \verb'\etal' macro provided, then you need not worry about double periods when used at the end of a sentence as in Alpher \etal.
However, use it only when there are three or more authors.
Thus, the following is correct:
   ``Frobnication has been trendy lately.
   It was introduced by Alpher~\cite{Alpher02}, and subsequently developed by
   Alpher and Fotheringham-Smythe~\cite{Alpher03}, and Alpher \etal~\cite{Alpher04}.''

This is incorrect: ``... subsequently developed by Alpher \etal~\cite{Alpher03} ...'' because reference~\cite{Alpher03} has just two authors.

\begin{figure*}
  \centering
  \begin{subfigure}{0.68\linewidth}
    \fbox{\rule{0pt}{2in} \rule{.9\linewidth}{0pt}}
    \caption{An example of a subfigure.}
    \label{fig:short-a}
  \end{subfigure}
  \hfill
  \begin{subfigure}{0.28\linewidth}
    \fbox{\rule{0pt}{2in} \rule{.9\linewidth}{0pt}}
    \caption{Another example of a subfigure.}
    \label{fig:short-b}
  \end{subfigure}
  \caption{Example of a short caption, which should be centered.}
  \label{fig:short}
\end{figure*}


==> Competition/2_formatting.tex <==
\section{Methodology}
\label{sec:formatting}

%-------------------------------------------------------------------------
\subsection{Visual Network}
Facial expressions in videos carry information pertinent to both appearance and temporal dynamics. Efficient modeling of these spatial and temporal cues plays a crucial role in extracting discriminant and robust features, which in-turn improves the overall system performance. State-of-the-art performance is typically achieved using 2D-CNN in combination with Recurrent Neural Networks (RNN) to capture the effective latent appearance representation, along with temporal dynamics \cite{7904596}. Several approaches have been explored for dimensional facial ER based on 2D-CNNs and LSTMs \cite{5740839,WOLLMER2013153} and 3D CNNs \cite{9667055,10095234,10005783}. In this work, we have used Resnet-50 pretrained on MS-CELEB-M dataset, which is further finetuned on FER+ dataset. Temporal Convolutional Networks (TCN) was found to be efficient in capturing the long term temporal dependencies \cite{9607460}. Therefore, we have used TCN in conjunction with Resnet-50 to obtain the spatiotemporal features of the visual modality.


\subsection{Audio Network}
The para-lingual information of vocal signals conveys significant information on the emotional state of a person. Even though vocal ER has been widely explored using conventional handcrafted features, such as Mel-frequency cepstral coefficients (MFCCs) \cite{Sethu2015}, there has been a significant improvement over recent years with the introduction of DL models. Though deep vocal ER models can be explored using spectrograms with 2D-CNNs, as
well as raw A signal with 1D-CNNs, spectrograms are
found to carry significant para-lingual information pertaining to the affective state of a person. Therefore, we consider spectrograms in the proposed framework along with 2D-CNN models to extract A features. In particular, we have explored VGG architecture to extract the audio embeddings \cite{45611}, which is further fed to TCN networks to model the temporal relationships across the frame-level audio embeddings.

\subsection{Recursive Joint Cross Attention (RJCA)}

Inspired by the performance of \cite{praveen2023recursive}, we have used their approach as a baseline to evaluate the proposed gated joint attention model. This section briefly discusses their approach, the recursive joint cross-attention model as a preliminary for our work. 
%We have developed an audio visual fusion joint attention model, where the attention is applied on A and V features in a recursve fahion in ordwer to efficeintly capture the intra and inter modeal relationships across Audio and Visual modalities. Specifically, we have exprelored recursive mechanism which helps in not only refininf the featurs but also acts a regularizer to improve the performncen of the ystem. %In this work we have focused on effectively capturing the intra and inter modal relationships across the audion and visual freature vectorts, while still still refining the fetures in a recursiove fahion. Specifically, we have attempted to analyze the cohernecey of audio and vidual features within a video subsequeunce of consecutive video clips by leveraging the complementary relationship across the audio and visual modalities while effectively preserving the intra modal temporal dynamics using LSTMs as well as joint representation in the fusion model. In order to effectively learn the intra and inter-modal complementary relationships, a joint cross-attention mechanism is deployed in a recursive fashion. Recursively training the joint cross-attention module helps to efficiently capture the complementary relationship and obtain more refined feature representations.   
Given the audio and visual feature vectors ${\boldsymbol X}_{\mathbf a}$ and ${\boldsymbol X}_{\mathbf v}$ for a video sub-sequence $\boldsymbol S$, the joint feature vectors are obtained by concatenating the audio and visual feature vectors, which is given by  
\begin{equation}
 {\boldsymbol J} = [{\boldsymbol X}_{\mathbf a} ; {\boldsymbol X}_{\mathbf v}] \in\mathbb{R}^{d\times L}
\end{equation}
where $d = {d_a} + {d_v}$ denotes the feature dimension of concatenated features. %By introducing the joint feature representation in the cross-attention module, the feature vectors of each modality learn from themselves as well as other modalities. 
The correlation between the joint feature vectors $\boldsymbol{J}$ and the individual feature vectors are estimated to measure the semantic relevance within the same modality as well as other modalities, which is obtained as 
\begin{align}
   \boldsymbol C_{\mathbf a}= \tanh \left(\frac{{\boldsymbol X}_{\mathbf a}^T{\boldsymbol W}_{\mathbf j \mathbf a}{\boldsymbol J}}{\sqrt d}\right) \\
   \boldsymbol C_{\mathbf v}= \tanh \left(\frac{{\boldsymbol X}_{\mathbf v}^T{\boldsymbol W}_{\mathbf j \mathbf v}{\boldsymbol J}}{\sqrt d}\right)
\end{align}
where ${\boldsymbol W}_{\mathbf j \mathbf a}, {\boldsymbol W}_{\mathbf j \mathbf v} \in\mathbb{R}^{L\times L} $ represents learnable weight matrices, $T$ denotes transpose operation, $\boldsymbol C_{\mathbf a}$ and $\boldsymbol C_{\mathbf v}$ denotes the joint correlation matrices of audio and visual modalities respectively. %The higher correlation coefficient of the joint correlation matrices means that the corresponding features are highly relevant to each other. 
Now the attention maps of audio and visual modalities are estimated as 
\begin{align}
\boldsymbol H_{\mathbf a}=ReLu(\boldsymbol X_{\mathbf a} \boldsymbol W_{\mathbf c \mathbf a} {\boldsymbol C}_{\mathbf a})
\\
\boldsymbol H_{\mathbf v}=ReLu(\boldsymbol X_{\mathbf v} \boldsymbol W_{\mathbf c \mathbf v} {\boldsymbol C}_{\mathbf v})
\end{align}
%Similarly, the joint correlation matrix for V features are given by: 
%The joint correlation matrices captures the semantic relevance across the A and V modalities as well as within the same modalities among consecutive video clips, which helps in effectively leveraging intra and inter modal relationships. % are effectively captured. %Higher correlation coefficient of the joint correlation matrices $\boldsymbol C_{\mathbf a}$ and $\boldsymbol C_{\mathbf v}$ shows that the corresponding samples are strongly correlated within the same modality as well as other modality. %modality, and the combined A-V feature representation are strongly correlated. 
%Therefore, the proposed approach is able to efficiently leverage the complementary nature of A and V modalities (i.e., inter-modal relationship) as well as intra-modal relationships, thereby improving the performance of the system. 
%After computing the joint correlation matrices, the attention weights of A and V modalities are estimated. 
%Since the dimensions of joint correlation matrices ($\mathbb{R}^{d_a\times d}$) and the features of corresponding modality ($\mathbb{R}^{L\times d_a}$) differ, we rely on a different learnable weight matrices corresponding to features of the individual modalities, and the corresponding joint correlation matrices, in order to compute attention weights of the modalities. 
%For the A modality, the joint correlation matrix $\boldsymbol C_{\mathbf a}$ and the corresponding A features ${\boldsymbol X}_{\mathbf a}$ are combined using the learnable weight matrices $\boldsymbol W_{\mathbf c \mathbf a}$ to compute the attention weights of A modality, which is given by 
%\begin{equation}
%$\boldsymbol H_{\mathbf a}=ReLu(\boldsymbol X_{\mathbf a} \boldsymbol W_{\mathbf c \mathbf a} {\boldsymbol C}_{\mathbf a})$
%\end{equation}
where ${\boldsymbol W}_{\mathbf c \mathbf a} \in\mathbb{R}^{{d_a}\times {d_a}}, {\boldsymbol W}_{\mathbf c \mathbf v} \in\mathbb{R}^{{d_v}\times {d_v}}$ denotes learnable weight matrices and ${\boldsymbol H}_{\mathbf a}, {\boldsymbol H}_{\mathbf v}$ represents the attention maps of the audio and visual modalities respectively. 
%Similarly, the attention maps ($\boldsymbol H_{\mathbf v}$) of V modality are obtained as 
%\begin{equation}
%$\boldsymbol H_{\mathbf v}=ReLu(\boldsymbol X_{\mathbf v} \boldsymbol W_{\mathbf c \mathbf v} {\boldsymbol C}_{\mathbf v})$
%\end{equation}
%where ${\boldsymbol W}_{\mathbf c \mathbf v} \in\mathbb{R}^{{d_v}\times {d_v}} $.

Then, the attention maps are used to compute the attended features of audio and visual modalities as: 
\begin{align}
{\boldsymbol X}_{\mathbf a \mathbf t \mathbf t, \mathbf a} = \boldsymbol H_{\mathbf a} \boldsymbol W_{\mathbf h \mathbf a} + \boldsymbol X_{\mathbf a}
\\
{\boldsymbol X}_{\mathbf a \mathbf t \mathbf t, \mathbf v} = \boldsymbol H_{\mathbf v} \boldsymbol W_{\mathbf h \mathbf v} + \boldsymbol X_{\mathbf v}  
\end{align}
where $\boldsymbol W_{\mathbf h \mathbf a}, \boldsymbol W_{\mathbf h \mathbf v} \in\mathbb{R}^{d\times {d_a}}$ represents learnable weights matrices and ${\boldsymbol X}_{\mathbf a \mathbf t \mathbf t, \mathbf a}, {\boldsymbol X}_{\mathbf a \mathbf t \mathbf t, \mathbf v}$ denotes the attended features of audio and visual modalities respectively, which is again fed to the joint cross attention model in a recursive fashion, shown as 
%and $\boldsymbol W_{\mathbf h \mathbf v} \in\mathbb{R}^{d\times {d_v}}$ denote the learnable weight matrices for A and V respectively.
%After obtaining the attended features they are fed again to the joint cross attentional model to compute the new A and V feature representations as:
\begin{align}
{\boldsymbol X}_{\mathbf a \mathbf t \mathbf t, \mathbf a}^{(t)} = \boldsymbol H_{\mathbf a}^{(t)} \boldsymbol W_{\mathbf h \mathbf a}^{(t)} + \boldsymbol X_{\mathbf a}^{(t-1)}
\\
{\boldsymbol X}_{\mathbf a \mathbf t \mathbf t, \mathbf v}^{(t)} = \boldsymbol H_{\mathbf v}^{(t)} \boldsymbol W_{\mathbf h \mathbf v}^{(t)} + \boldsymbol X_{\mathbf v}^{(t-1)}  
\end{align}
where $\boldsymbol W_{\mathbf h \mathbf a}^{(t)},\boldsymbol W_{\mathbf h \mathbf v}^{(t)} \in\mathbb{R}^{d\times {d_a}}$ denote the learnable weight matrices of $t^{th}$ iteration and ${\boldsymbol X}_{\mathbf a \mathbf t \mathbf t, \mathbf a}^{(t)}, {\boldsymbol X}_{\mathbf a \mathbf t \mathbf t, \mathbf v}^{(t)}$ denote the attended features of audio and visual modalities after $t$ iterations respectively.
%for A and V respectively. %After $t$ iterations, the final attended features are concatenated to obtain multi-modal features as
%\begin{equation}
% {\boldsymbol X}_{\mathbf a \mathbf t \mathbf t} = [{\boldsymbol X}_{\mathbf a \mathbf t \mathbf t, \mathbf a}^{(t)} ; {\boldsymbol X}_{\mathbf a \mathbf t \mathbf t, \mathbf v}^{(t)}] 
%\end{equation}
%Finally, the attended A and V features after $t$ iterations are further concatenated and fed to BLSTM to obtain the temporal dependencies within the refined A-V feature representations, which are fed to fully connected layers for final prediction. %for the prediction of valence or arousal. 
\subsection{Gated Recursive Joint Cross Attention Model}
Though audio and visual modalities are expected to be complementary to each other \cite{9758834}, they may not always be compatible with each other \cite{9552921}. %For instance, if one of the modalities is highly corrupted or noisy due to extreme background noise or clutter, it may potentially deteriorate the fused feature representation \cite{9053012}. 
Therefore, we present a gated attention mechanism to adaptively fuse the audio and visual features, based on the compatibility of the modalities with each other i.e., the gated attention emphasizes the cross-attended features when the features exhibit a strong complementary relationship, otherwise non-attended features. By adaptively emphasizing the most relevant features, the proposed model can handle both strong and weak complementary relationships, thereby improving the performance of the system. %The proposed model can also be adapted to other fusion mechanisms based on cross-modal interactions since the adaptive gating attention model is agnostic to the fusion mechanism being deployed. 
Given the attended features of multiple iterations and non-attended features from audio and visual modalities, we design a gating layer using a fully connected layer for every iteration of each modality separately to obtain the attention weights for the attended and non-attended features, which are given by 
\begin{align}
{\boldsymbol W}_{go,v}^{(t)} = {\boldsymbol X}_{att,v}^{(t)} \boldsymbol W_{gl,v}^{(t)}
\quad  \text{and} \quad
{\boldsymbol W}_{go,a}^{(t)} = {\boldsymbol X}_{att,a}^{(t)} \boldsymbol W_{gl,a}^{(t)}
\end{align}
where $\boldsymbol W_{gl,a}^{(t)} \in\mathbb{R}^{d_a\times 2}$, $\boldsymbol W_{gl,v}^{(t)}\in\mathbb{R}^{d_v\times 2}$ are the learnable weights of the gating layers of $t$-th iteration and $\boldsymbol W_{go,a}^{(t)} \in\mathbb{R}^{L\times 2}$, $\boldsymbol W_{go,v}^{(t)} \in\mathbb{R}^{L\times 2}$ are outputs of gating layers of audio and visual modalities of $t$-th respectively. In order to obtain probabilistic attention scores, the output of the gating layers is activated using a softmax function with a small temperature $T$, as given by 
\begin{align}
{\boldsymbol G}_{a}^{(t)}
=\frac{ e^{{\boldsymbol W}_{go,a}^{(t)}/T}}{\overset{ K}{\underset{ k\boldsymbol=1}{\sum}} e^{{\boldsymbol W}_{go,a}^{(t)}/T}}    
\quad  \text{and} \quad
{\boldsymbol G}_{v}^{(t)}
=\frac{ e^{{\boldsymbol W}_{go,v}^{(t)}/T}}{\overset{K}{\underset{ k\boldsymbol=1}{\sum}} e^{{\boldsymbol W}_{go,v}^{(t)}/T}}    
\end{align}
where $\boldsymbol {G}_{a}^{(t)} \in\mathbb{R}^{L\times 2}, \boldsymbol {G}_{v}^{(t)}\in\mathbb{R}^{L\times 2}$ denotes the probabilistic attention scores of audio and visual modalities. $K$ denotes the number of output units of the gating layer, which is $2$. In our experiments, we have empirically set the value of $T$ to 0.1. %The weights of the attended and non-attended features are obtained from the probabilistic attention scores of the gating layers from audio and visual modalities, respectively as


The probabilistic attention scores of the gating layer help estimate the relevance of attended features of iteration $t$ and iteration (previous) $(t-1)$ for the accurate prediction of valence and arousal. The two columns of $\boldsymbol G_a^{(t)}$ correspond to the probabilistic attention scores of iteration $t$ (first column) and iteration $t-1$ (second column). To multiply with the corresponding feature vectors, each column is replicated to match the dimension of the corresponding feature vectors, which is denoted by $\boldsymbol G_{a0}^{(t)}$, $\boldsymbol G_{a1}^{(t)}$ and $\boldsymbol G_{v0}^{(t)}$, $\boldsymbol G_{v1}^{(t)}$ for audio and visual modalities respectively. Now, the replicated attention scores  %The columns of the matrices ${\boldsymbol W}_{\mathbf g \mathbf a}, {\boldsymbol W}_{\mathbf g \mathbf v}, {\boldsymbol W}_{\mathbf a \mathbf t \mathbf t,\mathbf g \mathbf v}$ and ${\boldsymbol W}_{\mathbf a \mathbf t \mathbf t,\mathbf g \mathbf v}$ are replicated to match the dimension of the original feature vectors. 
%The probabilistic attention scores obtained from the gated attention 
are multiplied with the corresponding features of iteration $t$ and $(t-1)$ of the respective modalities, which is further fed to the ReLU activation function as: 
\begin{align}
%\begin{equation}
{\boldsymbol X}_{att,gv}^{(t)} = \text{ReLU}({\boldsymbol X}_{att,v}^{(t-1)} \otimes \boldsymbol G_{v0}^{(t)} + {\boldsymbol X}_{att,v}^{(t)} \otimes \boldsymbol G_{v1}^{(t)}) \\ 
%\end{equation}   
%\vspace{-10mm}
%\begin{equation}
{\boldsymbol X}_{att,ga}^{(t)} = \text{ReLU}({\boldsymbol X}_{att,a}^{(t-1)} \otimes \boldsymbol G_{a0}^{(t)} + {\boldsymbol X}_{att,a}^{(t)} \otimes \boldsymbol G_{a1}^{(t)})  
\end{align}
where $\otimes$ denotes element-wise multiplication. ${\boldsymbol X}_{att,ga}^{(t)}$ and ${\boldsymbol X}_{att,gv}^{(t)}$ denote the attended features of audio and visual modalities of iteration $t$ respectively. % obtained from DCA model, which is further %${\boldsymbol X}_{\mathbf a\mathbf t\mathbf t\boldsymbol,\mathbf g \mathbf v}$ and $ {\boldsymbol X}_{\mathbf a\mathbf t\mathbf t\boldsymbol,\mathbf g \mathbf a}$ are 
%concatenated to obtain the A-V feature representations ${\boldsymbol X}_{att,g}$, followed by regression layers to get final predictions. %as given by 

To further enhance the flow of information across all the iterations of the RJCA model, we employ a high-level gating mechanism that can obtain semantic features by controlling the flow of information across the gated features of all iterations. Given the features obtained from the gating layers of every iteration, the final features for audio and visual modalities can be obtained as 
\begin{align}
{\boldsymbol X}_{att,ga}^{(f)} = \text{ReLU}({\overset{M}{\underset{ t\boldsymbol=1}{\sum}} {\boldsymbol X}_{att,ga}^{(t)}} \otimes \boldsymbol G_{vt}^{(f)}) \\
{\boldsymbol X}_{att,gv}^{(f)} = \text{ReLU}({\overset{M}{\underset{ t\boldsymbol=1}{\sum}} {\boldsymbol X}_{att,gv}^{(t)}} \otimes \boldsymbol G_{vt}^{(f)})
\end{align}
where $M$ denotes the number of iterations, ${\boldsymbol X}_{att,ga}^{(f)}$ and ${\boldsymbol X}_{att,gv}^{(f)}$ denote the final attended features of audio and visual modalities respectively, $\boldsymbol G_{at}^{(f)}$ and $\boldsymbol G_{vt}^{(f)}$ denote the gating outputs of the final gating layer. The final attended features of audio and visual modalities are fed to Multi-Layer Perceptron (MLP) for final predictions of valence and arousal.






\section{Experimental Setup}
\subsection{Dataset}
Affwild2 is the largest database in the field of affective computing captured in-the-wild conditions. It is composed of 594 videos collected from YouTube, all captured in-the-wild. Sixteen of these video clips display two subjects, both of which have been annotated. The annotations are provided by four experts using a joystick and the final annotations are obtained as the average of the four raters. In total, there are 2, 993, 081 frames with 584 subjects, out of which 277 are male and 178 female. The annotations for valence and arousal are provided continuously in the range of [-1, 1]. The dataset is split into the training, validation and test sets. The partitioning is done in a subject independent manner,
so that every subject’s data will present in only one subset. The partitioning produces 356, 76, and 162 train, validation and test videos respectively.
\begin{table*}
%\scriptsize
\setlength{\tabcolsep}{4pt}
\renewcommand{\arraystretch}{1.25}
    \centering
    \caption{ \textbf{CCC of the proposed approach compared to state-of-the-art methods for A-V fusion on the Affwild2 development set. }}
    \label{Comparison with state-of-the-art for Affwild2 validation}
    \begin{tabular}{|l|l||c|c|c|c|c|c||c|c|c|} 
	\hline
	 \textbf{Method}  & \textbf{Backbones} &  \multicolumn{3}{|c|}{\textbf{Valence}} & \multicolumn{3}{|c||}{\textbf{Arousal}}  \\ \cline{3-8}
	 & &\textbf{Audio}  & \textbf{Visual}  & \textbf{Fusion}  & \textbf{Audio} & \textbf{Visual} & \textbf{Fusion}\\
	 \hline
 	 %\multicolumn{7}{|c|}{\textbf{Weakly-Supervised}} \\
	\hline
    Kuhnke et al. \cite{9320301}  & A: Resnet18; V: R(2plus1)D & 0.351 & 0.449 & 0.493 & 0.356 & 0.565 & 0.604 \\
	\hline
    Zhang et al. \cite{9607460}  & A: VGGish; V: Resnet50 & - & 0.405 & 0.457 & - &  0.635  & 0.645 \\
    \hline
	 Rajasekhar et al. \cite{9667055}  & A: Resnet18; V: I3D & 0.351  & 0.417 & 0.552 & 0.356 & 0.539 & 0.531\\ 
	\hline 
	Joint Cross-Attention \cite{Praveen_2022_CVPR} & A: Resnet18; V: I3D-TCN & 0.351  & 0.417 & 0.663 & 0.356 & 0.539 & 0.584\\ 
	\hline
	Recursive Joint Cross-Attention \cite{Praveen_2022_CVPR} & A: Resnet18; V: I3D-TCN & 0.351  & 0.417 & 0.721 & 0.356 & 0.539 & 0.694\\ 
	\hline
    GRJCA (Ours) & A: VGGish; V: Resnet-50 & -  & 0.405 & 0.623 & - & 0.635 & 0.660\\ 
	\hline
\end{tabular}
     %\vspace{-8mm}
\end{table*}
\subsection{Implementation Details}
In this section, we provide the implementation details of the system submitted for ABAW8 competition \cite{Kollias2025,kolliasadvancements}. For the V modality, we have used the cropped and aligned images provided by the challenge organizers. For the missing frames in the V modality, we have considered black frames (i.e., zero pixels). Faces are resized to 48x48 to be fed to the Resnet-50 network. The subsequence length of the videos are considered to be 300. To regularize the network, dropout is used with p = 0.8 on the linear layers. Data augmentation is performed on the training data by random cropping, which produces scale in-
variant model. The number of epochs is set to 100, and early stopping is used to obtain weights of the best network.

For the A modality, the vocal signal is extracted from the corresponding video, and resampled to 44100Hz, which is further segmented to short vocal segments corresponding a
sub-sequence of 256 frames of the V network. The spectrogram is obtained using Discrete Fourier Transform (DFT) of length 1024 for each short segment, where the window length is considered to be 20 msec and the hop length to be 10 msec. Following aggregation of short-time spectra, we obtain the spectrogram of 64 x 107 corresponding to each sub-sequence of the V modality. Now a normalization step is performed on the obtained spectrograms. The spectrogram is converted to log-power-spectrum, expressed in dB. Finally, mean and variance normalization is performed on the spectrogram. Now the obtained spectrograms are fed
to the VGG to obtain the A features. 

Similar to that of \cite{10208757}, we also fine-tuned the visual backbone along with the fusion network in a gradual fashion by gradually releasing the layers of Resnet-50 backbones. For the fusion network, the initial weights of the cross-attention matrix is initialized with Xavier method [4], and the weights are updated using Adam optimizer. The initial learning rate is set to be 0.0001 and batch size is fixed to be 12. Also, dropout of 0.5 is applied on the attended A-V features and weight decay of 0.0005 is used for all the experiments. The repetitive warm-up is carried out until epoch$=$5. After which the ReduceLROnPlateau takes over to update the learning rate. It gradually drops the learning rate in a factor of $0.1$ should no higher validation CCC appears for a consecutive 5 epochs. Due to the spontaneity of the expressions, the annotations are also found to be highly stochastic in nature. 6-fold cross-validation is performed and the best folds that show higher validation scores are used to obtain the test set predictions.

\section{Results}
In this work, we have provided the results of our approach along with some of the relevant methods of previous challenges of ABAW \cite{kollias2023abaw2,kollias2023multi,kollias2023abaw,kollias2022abaw,kollias2021analysing,kollias2021affect,kollias2021distribution,kollias2020analysing,kollias2019expression,kollias2019deep,kollias2019face,zafeiriou2017aff,kollias20246th,kollias20247th,kollias2024distribution}. Table \ref{Comparison with state-of-the-art for Affwild2 validation} shows our comparative results against relevant state-of-the-art A-V fusion models on the Affwild2 validation set. Kuhnke et al. \cite{9320301} used 3D-CNNs, where the R(2plus1)D model is used for the V modality, and the Resnet18 is used for the A modality. However, they use additional masks for the V modality and annotations of other tasks to refine the annotations of valence and arousal. They further perform simple feature concatenation without any specialized fusion model to predict valence and arousal. Therefore, the performance with fusion was not significantly improved over the uni-modal performance. Zhang et al. \cite{9607460} explored the leader-follower attention model for fusion and showed minimal improvement in fusion performance over uni-modal performances. Though they have shown significant performance for arousal than valence, it is mostly attributed to the V backbone. Similar to that of \cite{9607460}, we also follow the same backbones for the audio, visual modalities. By deploying the gating mechanism, we are able to efficiently handle the weak complementary relationships to improve the performance of the system. Even with vanilla cross-attentional fusion \cite{9667055}, the fusion performance for valence has been improved better than that of \cite{9607460} and \cite{9320301}. By deploying joint representation into the cross attentional fusion model, the fusion performance of valence has been significantly improved further. In this work, we further extended our previous work \cite{10095234} by introducing gating mechanism to deal with the weak complementary relationships across audio and visual modalities. 

It is worth mentioning that we did not use any external dataset or features from multiple backbones for A and V modalities. The performance of the proposed approach is solely attributed to the efficacy of our fusion model. We observed that the fusion performance has been significantly improved over the uni-modal performances, especially for valence. We have shown that effectively leveraging the inter-modal relationships by handling weak complementary relationships can significantly imrpve the performance of the fusion model. The proposed fusion model can be further improved using the fusion of multiple audio and visual backbones either through feature-level or decision-level fusion similar to that of the winner of the challenge \cite{Situ-RUCAIM3}.





==> Competition/3_finalcopy.tex <==
\section{Final copy}

You must include your signed IEEE copyright release form when you submit your finished paper.
We MUST have this form before your paper can be published in the proceedings.

Please direct any questions to the production editor in charge of these proceedings at the IEEE Computer Society Press:
\url{https://www.computer.org/about/contact}.
